Dispersion Analysis of Finite Difference and Discontinuous Galerkin Schemes for Maxwell's Equations in Linear Lorentz Media

In this paper, we consider Maxwell's equations in linear dispersive media described by a single-pole Lorentz model for electronic polarization. We study two classes of commonly used spatial discretizations: finite difference methods (FD) with arbitrary even order accuracy in space and high spatial order discontinuous Galerkin (DG) finite element methods. Both types of spatial discretizations are coupled with second order semi-implicit leap-frog and implicit trapezoidal temporal schemes studied in our previous research [5,6]. By performing detailed dispersion analysis for the semi-discrete and fully discrete schemes, we obtain rigorous quantification of the dispersion error for Lorentz dispersive dielectrics. In particular, comparisons of dispersion error can be made taking into account the model parameters, and mesh sizes in the design of the two types of schemes. The results for the numerical dispersion analysis can guide us in the optimal choice of discretization parameters for the more complicated and nonlinear models. The numerical dispersion analysis of the fully discrete FD and DG schemes, for the dispersive Maxwell model considered in this paper, clearly indicate the dependence of the numerical dispersion errors on spatial and temporal discretizations, their order of accuracy, mesh discretization parameters and model parameters. The results obtained here cannot be arrived at by considering discretizations of Maxwell's equations in free space. In particular, our results contrast the advantages and disadvantages of using high order FD or DG schemes and leap-frog or trapezoidal time integrators over different frequency ranges using a variety of measures of numerical dispersion errors. Finally, we highlight the limitations of the second order accurate temporal discretizations considered.

==> Ack.tex <==
\section{Acknowledgements}
The authors would like to thank ICERM's {\it Collaborate\@ ICERM} program as well as the {\it Research in Pairs} program at MFO, Oberwolfach in Germany for their support of co-authors Bokil, Cheng and Li. The authors would also like to thank NSF...

==> conclude.tex <==
\section{Conclusions and Future Directions}

In this paper, we developed new high spatial order FDTD methods that are second order accurate in time for a nonlinear Maxwell model in one spatial dimension. The nonlinear Maxwell model includes an instantaneous cubic Kerr nonlinearity as well as both linear and nonlinear Lorentz dispersion, where the nonlinear Lorentz dispersion arises due to Raman scattering. The fully discrete FDTD methods are energy stable and we have computed theoretically the Courant stability limits for arbitrary spatial orders for the leap-frog schemes. The trapezoidal methods are shown to be unconditionally stable. The second order temporal accuracy of the methods is generated by developing new time discretizations that provide for fully discrete energy identities that respect  the continuum energy identities.

In future work, we will extend our results to two and three dimensional spatial models. 

 
